Ditto: Elastic Confidential VMs with Secure and Dynamic CPU Scaling

Confidential Virtual Machines (CVMs) are a type of VMbased Trusted Execution Environments (TEEs) designed to enhance the security of cloud-based VMs, safeguarding them even from malicious hypervisors. Although CVMs have been widely adopted by major cloud service providers, current CVM designs face significant challenges in runtime resource management due to their fixed capacities and lack of transparency. These limitations hamper efficient cloud resource management, leading to increased operational costs and reduced agility in responding to fluctuating workloads. This paper introduces a dynamic CPU resource management approach, featuring the novel concept of "Elastic CVM. This approach allows for hypervisor-assisted runtime adjustment of CPU resources using a specialized vCPU type, termed Worker vCPU. This new approach enhances CPU resource adaptability and operational efficiency without compromising security. Additionally, we introduce a Worker vCPU Abstraction Layer to simplify Worker vCPU deployment and management. To demonstrate the effectiveness of our approach, we have designed and implemented a serverless computing prototype platform, called Ditto. We show that Ditto significantly improves performance and efficiency through finergrain resource management. The concept of "Elastic CVM" and the Worker vCPU design not only optimize cloud resource utilization but also pave the way for more flexible and cost-effective confidential computing environments.

==> backup.tex <==
\subsection{Protection Schemes in SEV}

\bheading{Reverse Map Table (RMP).} Reverse Map Table (RMP) is a data structure used by SEV to protect the integrity of the memory mapping information. Specifically, in SEV, a 2-level nested page table (NPT) is used to store the mapping information between the guest virtual address (\textit{gVA}) and the guest physical address (\textit{gPA}), as well as the mapping between \textit{gPA} and the system physical address (\textit{sPA}). While the first level NPT, \aka, guest page table, is completely maintained and protected by CVM, the second level NPT, \aka, host page table, is maintained by the hypervisor and remains unprotected. To prevent a malicious hypervisor from  and protect against attacks.  
[add a figure][if we decide to run only in SEV-ES, then give up this section. Thus, I will work on other sections first.]



\bheading{Emulated interrupt.} In a virtualized environment, interrupt signals are managed using software-emulated APIC or x2APIC interfaces. 

\bheading{Restricted Injection Mode.} When a vCPU is configured to run in this mode, the hypervisor is not allowed to inject interrupts directly to the vCPU. Instead, the CPU hardware only allows the hypervisor to inform the vCPU that some interrupts are pending through a new defined exception, called \texttt{\#HV} exception. The \texttt{\#HV} exception acts like a doorbell and the vCPU can then re-scan the event queue located in a shared memory for pending interrupt information.

\bheading{Alternate Injection Mode.} A vCPU running in this mode allows standard virtual interrupt queuing and injection. However, the injection can only be made by the confidential VM itself, e.g., another vCPU running in VMPL0. 


\bheading{I/O in CVM.}

\bheading{Remote attestation.} 

\bheading{Live migration.}



\bheading{Secure CVM and hypervisor coordination.}
To address the aforementioned challenges, \sysname introduces and follows a \textit{secure CVM and hypervisor coordination principle}. In this approach, the CVM's kernel and boot loader assist the hypervisor in adjusting the number of vCPUs, while ensuring that neither the CVM nor the hypervisor compromises security or performance.

To efficiently utilize echo vCPU and achieving seamless suspension is another challenge within CVM.
From a performance perspective, effective adjustment requires the OS and applications to promptly recognize and utilize newly added vCPUs. This usually requires significant changes to the OS and applications or necessary a VM reboot. Conversely, they also need to efficiently manage vCPU removal when demand decreases to conserve resources.

% Besides, even if a vCPU is allowed to be added into the CVM, both the OS and the application must be aware of this and act promptly to fully utilise the newly added vCPU. The OS must setup the vCPU and schedule tasks to it; The application must know the vCPU exists and spawn a new thread for the vCPU. Moreover, when the load decreases, the newly added vCPU needs to be removed to return to save the resource. That also means both the application and the OS needs to be aware of this at runtime.

In this context, the hypervisor is responsible for the dynamic adjustment of vCPU numbers, 

ensuring that these changes remain transparent to the CVM owner during runtime. In practical cloud environments, \sysname can act more fast as no approve from CVM owner are needed to adjust vCPU number and can be seamlessly integrated with existing confidential serverless computing platforms or applications that adhere to the producer-consumer model.

adapting this vCPU adjustment, while such design is already enough for CVM owner to manage CPU resources itself.

Therefore, in our system, we consider an \textit{\textbf{auto-regulated}} echo vCPU management design, where the management of echo vCPUs is offloaded to the hypervisor. This hypervisor-controlled approach, although more specific, is a preferred management way in cloud computing, enabling a faster response in managing echo vCPUs without worrying about resource management.

In this paper, we introduce \sysname, a system that enables secure, rapid, and auto-regulated vCPU adjustment for CVMs.

To ensure that the security of the CVM is not compromised if the untrustworthy hypervisor maliciously puts echo vCPUs to sleep or wakes them up, the tasks executed on these echo vCPUs are designed to be stateless. This design is common in applications following a producer-consumer model, such as Nginx and Redis worker threads. A simple protocol can also be setup between the echo vCPUs and the hypervisor, specifying the conditions under which the hypervisor should wake up or put the echo vCPUs to sleep.
During runtime, the hypervisor can wake up echo vCPUs in response to specific events or high vCPU utilization, and put them back to sleep when they are no longer needed. Throughout this process, the states of the echo vCPUs and other aspects of the CVM remain hidden from the hypervisor, ensuring the overall security of the system.
